Randomized polynomial-time equivalence between determinant and trace-IMM equivalence tests

Equivalence testing for a polynomial family {g_m} over a field F is the following problem: Given black-box access to an n-variate polynomial f(x), where n is the number of variables in g_m, check if there exists an A in GL(n,F) such that f(x) = g_m(Ax). If yes, then output such an A. The complexity of equivalence testing has been studied for a number of important polynomial families, including the determinant (Det) and the two popular variants of the iterated matrix multiplication polynomial: IMM_{w,d} (the (1,1) entry of the product of d many w $\times$ w symbolic matrices) and Tr-IMM_{w,d} (the trace of the product of d many w $\times$ w symbolic matrices). The families Det, IMM and Tr-IMM are VBP-complete, and so, in this sense, they have the same complexity. But, do they have the same equivalence testing complexity? We show that the answer is 'yes' for Det and Tr-IMM (modulo the use of randomness). The result is obtained by connecting the two problems via another well-studied problem called the full matrix algebra isomorphism problem (FMAI). In particular, we prove the following: 1. Testing equivalence of polynomials to Tr-IMM_{w,d}, for d$\geq$ 3 and w$\geq$ 2, is randomized polynomial-time Turing reducible to testing equivalence of polynomials to Det_w, the determinant of the w $\times$ w matrix of formal variables. (Here, d need not be a constant.) 2. FMAI is randomized polynomial-time Turing reducible to equivalence testing (in fact, to tensor isomorphism testing) for the family of matrix multiplication tensors {Tr-IMM_{w,3}}. These in conjunction with the randomized poly-time reduction from determinant equivalence testing to FMAI [Garg,Gupta,Kayal,Saha19], imply that FMAI, equivalence testing for Tr-IMM and for Det, and the $3$-tensor isomorphism problem for the family of matrix multiplication tensors are randomized poly-time equivalent under Turing reductions.

==> figure_lie_algebra_matrices.tex <==
\begin{tikzpicture}
% CORNERS
\coordinate (a) at (0,0);
\coordinate (b) at ($(a) + (3,0)$);
\coordinate (c) at ($(a) + (3,-3)$);
\coordinate (d) at ($(a) + (0,-3)$);

\node at ($ (a) + (0.75,-0.75)$) [fill=white!100!] {\scriptsize $I_w\otimes M^T$};
\node at ($ (b) - (0.75, 0.75)$) [fill=white!100!] {\scriptsize $\mathbf{0}$};
\node at ($ (a) + (0.75, 0.75)$) [fill=white!100!] {\scriptsize $\mathbf{0}$};
\node at ($ (d) - (0.75,-0.75)$) [fill=white!100!] {\scriptsize $-I_w\otimes M$};

\draw (a) -- (b) -- (c) -- (d) -- (a);
\end{tikzpicture}

==> temporary_lemmas.tex <==
\section{Temporary}



%\begin{lemma}{\label{lemma:diag_distinct}}
%There is a diagonal matrix $D \in \GIMM$ with distinct entries.
%\end{lemma}
%\begin{lemma}{\label{lemma:char_poly_sq_free}}
%Let $L_1, \ldots, L_t$ be a basis of $\GIMM$ and $L = \sum_{i = 1}^{t} r_iL_i$ where $r_i \in_R S; S \subset \mathbb{F}; |S| = 2n^3$. Then the characteristic polynomial of $L$ is square free with probability at least $1 - \frac{1}{poly(n)}$.
%\end{lemma}

%\begin{claim}{\label{claim:invar_subspace_is_coordinate}}
% Let $\mathcal{U}$ be an invariant subspace of $\GIMM$. Then $\mathcal{U}$ is a coordinate subspace.
%\end{claim} 

\begin{proof}
     For a vector $\mathbf{u} = (u_1, \ldots, u_n) \in \mathcal{U}$. Let $S_\mathbf{u}$ be the set of all non zero coordinates of $\mathbf{u}$, i.e. $S_{\mathbf{u}} := \{ j : u_j \neq 0\  \textnormal{and}\  j \in [n] \}$ and $E_{\mathbf{u}} := \{e_j: j \in S_{\mathbf{u}} \}$ be the corresponding unit vectors.
     Further suppose $E: = \cup_{\mathbf{u} \in \mathcal{U}}E_{\mathbf{u}}$. To show that $\mathcal{U}$ is a coordinate subspace,it is sufficient to show that \textnormal{span}($E$) $= \mathcal{U}$. Clearly, $\mathcal{U} \subseteq \textnormal{span}(E)$. To complete the proof we show that $e_j \in \mathcal{U}$ whenever $j \in S_{\mathbf{u}}$ for some $\mathbf{u} \in \mathcal{U}$. \\ 
      By Lemma~\ref{lemma:diag_distinct}, there exists a diagonal matrix $D \in \GIMM$ with distinct entries $\lambda_1, \ldots, \lambda_n$. Hence, $D^i\mathbf{u} = \mathbf{u_i} = (\lambda_1^iu_1, \ldots , \lambda_n^iu_n) \in \mathcal{U}$ for all $i \in [n]$ and $D^0\mathbf{u} = \mathbf{u}_0 = \mathbf{u}$. Denote $|S_{\mathbf{u}}|$ as $m$. We use the fact that since $\lambda_1, \ldots , \lambda_n$ are distinct to argue that the vectors $\mathbf{u_0}, \ldots , \mathbf{u_{m-1}}$ are linearly independent as follows: Let $c_0, \ldots, c_{m-1} \in \F$ be such that $c_0\mathbf{u_0} + \ldots + c_{m-1}\mathbf{u_{m-1}} = \mathbf{0}$ and not all $c_0, \ldots, c_{m-1}$ are 0. In particular for each coordinate $j \in [1,n-1]$
     \begin{align*}
          u_j(c_0+c_1\lambda_j+ \ldots + c_{m-1}\lambda_j^{m-1})= 0
     \end{align*}
       
  Notice that each $\lambda_j$, $j \in S_{\mathbf{u}}$, is a solution of the equation $c_0+c_1\lambda+ \ldots + c_{m-1}\lambda^{m-1} = 0$. But a non zero degree $m-1$ univariate polynomial in $\lambda$ can have at most $m-1$ roots, implying that $c_0 = c_1 = \ldots = c_{m-1} = 0$.  \\ 
  Since $\mathbf{u}_0, \ldots, \mathbf{u}_{m-1} \in \textnormal{span}(E_{\mathbf{u}})$ and $\textnormal{dim(span(}\{ \mathbf{u}_0, \ldots, \mathbf{u}_{m-1} \})) = \textnormal{dim(\textnormal{span}(} E_{\mathbf{u}} )) = m$, we infer that $\textnormal{span(}\{ \mathbf{u}_0, \ldots, \mathbf{u}_{m-1} \}) = \textnormal{span(} E_{\mathbf{u}} ))$. Hence $e_j \in \mathcal{U}$ where $j \in S_{\mathbf{u}}$ for some $\mathbf{u} \in \mathcal{U}$.
\end{proof}

\subsection{Diagrams} 
\begin{figure}[h]
\centering
%\includegraphics[height=10cm, width = 10cm,keepaspectratio]{figures/hkR.jpg}
\input{figures/fig_a.tex}
\caption{The matrix $h_k(R)$}
\label{}
\end{figure}

\begin{figure}[h]
\centering
%\includegraphics[height=10cm, width = 10cm,keepaspectratio]{figures/hkR.jpg}
\input{figures/fig_b.tex}
\caption{The matrix $h_k(R)$}
\label{)}
\end{figure}

\begin{figure}[h]
\centering
%\includegraphics[height=10cm, width = 10cm,keepaspectratio]{figures/hkR.jpg}
\input{figures/fig_c.tex}
\caption{The matrix $h_k(R)$}
\label{)}
\end{figure}
\section{Algorthmic Preliminaries}{\label{section:alg_prelims}}
In this section, we state some well known algorithms without proof. 
\begin{enumerate}
    \item \label{fact:lie_alg_basis} \textbf{Given blackbox access to an $n$ variate, degree $d$ polynomial $f$, a basis for the Lie Algebra of a polynomial $f$ can be computed.} This has been elaborated in \cite{DBLP:conf/stoc/Kayal12} where they give an efficient randomized algorithm to compute a basis for the Lie Algebra of an $n$ variate, degree $d$ polynomial $f$ that has running time $poly(n,d,\beta)$ where $\beta$ is the bit length of the coefficients.
    
    \item \label{fact:univariate_factorization} \sloppy \textbf{Univariate Polynomial Factorization: } \cite{lenstra1982factoring} gave an efficient deterministic algorithm ($O(poly(n, \beta))$ time), where $\beta$ is bound on the bit length of the polynomial) to factorize a univariate polynomial of degree $n$ over $\mathbb{Q}$. There are efficient randomized algorithms ($O(poly(n, \log q))$ time) such as \cite{berlekamp1967factoring},\cite{cantor1981new} to factorize a degree $n$ univariate polynomial over some finite field $\F_q$. .
    
    \item \label{fact:null_space_basis}\textbf{Basis of the null spaces: }We can efficiently compute a basis for the null space of any matrix $A \in \F^{n \times n}$. Let $A'$ be the row reduced echeolon form of $A$. Then $\textnormal{null}(A) = \textnormal{null}(A')$. A basis for $\textnormal{null}(A')$ can be found by analyzing the equations $A'\mathbf{x} = 0$. It is easy to see that solving this system of equations by gaussian elimination will take $O(n^3)$ time. 
    
    \item \label{fact:closure_of_v}\textbf{Computing the closure of a vector:} 
    Let $\mathbf{v} \in \F^n$ and $\mathcal{L}$ be the vector space over $\F$ spanned by matrices $\{M_1, \ldots,$ $ M_k \} \in \F^{n \times n}$. By definition $\textnormal{span}(\mathbf{v}) \in \textnormal{closure}(\mathbf{v})$. If $\mathbf{u} \in \textnormal{closure}(\mathbf{v})$ then $M_i\cdot\mathbf{u} \in \textnormal{closure}(\mathbf{v})$ for each $i \in [k]$.  Algorithm~\ref{alg:closure_of_v} computes the closure of a vector $\mathbf{v}$ under the action of $\mathcal{L}$ using this idea. In the \textit{while} loop (steps 4-6), the algorithm executes steps 5 and 6 only if $\mathcal{V}^{(i-1)}$ is a strict subspace of $\mathcal{V}^{(i)}$. Since $\textnormal{dim}(\textnormal{closure}(\mathbf{v}) \leq n$, the algorithm terminates after at most $n$ iterations of the \textit{while} loop.
    \begin{algorithm}
\caption{Computing the closure of a vector $\mathbf{v}$ under the action of a space $\mathcal{L}$}
{\label{alg:closure_of_v}}
INPUT: $\mathbf{v} \in \F^n$ and a basis $\{M_1, \ldots, M_k \}$ of $\mathcal{L}$.\\
OUTPUT: Basis of the $\textnormal{closure}(\mathbf{v})$ under the action of $\mathcal{L}$.
\begin{algorithmic}[1]
\State $\mathcal{V}^{(0)} = \{\mathbf{v}$\}. Then $T_0 = \{\mathbf{v}\}$ is a basis of $\mathcal{V}^{(0)}$.
\State $\mathcal{V}^{(1)} = \textnormal{span}_{\F}(T_0 \cup \mathcal{L}\cdot T_0)$ and $T_1$ be a basis of $\mathcal{V}^{(1)}$.
\State i = 1
\While{$\mathcal{V}^{(i)} \neq \mathcal{V}^{(i-1)}$}
    \State i = i+1
    \State  $\mathcal{V}^{(i)} = \textnormal{span}_{\F}(T_{i-1} \cup \mathcal{L}\cdot T_{i-1})$ and $T_i$ be a basis of $\mathcal{V}^{(i)}$.
\EndWhile
\State Output $T_i$.
\end{algorithmic}
\end{algorithm}


    \item \label{fact:comparing_vector_spaces} \textbf{Checking if two  $n$ dimensional vector spaces $\mathcal{V}_1$ and $\mathcal{V}_2$ are equal:} Let $V_1$ be the matrix whose columns are the basis vectors of $V_1$. For $\mathcal{V}_1$ to be equal to $\mathcal{V}_2$ we require that for each basis vector $\mathbf{v}$ of $\mathcal{V}_2$, the system of linear equation $V_1\mathbf{x} = \mathbf{v}$ has a solution. Solving a system of linear equations can be done efficiently ($O(\textnormal{dim}(\mathcal{V}_1)^3)$ time). 
    
     \item \label{fact:set_multilinear_abp_reconstruction} \textbf{Set Multilinear ABP Reconstruction:} Recall from Chapter~\ref{chap:introduction} that an ABP is the $(1,1)$-th entry of $w \times w$ matrices $X_1, \ldots, X_d$ whose entries are linear forms in the variables. Let $\mathbf{x}_i$ denote the variables appearing in $X_i$. An ABP is said to \textnormal{set-multilinear} whenever $i \neq j$ implies $\mathbf{x}_i \cap \mathbf{x}_j = 
    \emptyset$ for all $i,j \in [d]$. The \textit{set-multilinear ABP reconstruction} problem is the following: Given a polynomial $f$, (re)construct a set-multilinear ABP that computes it. \cite{DBLP:conf/colt/KlivansS03} give an efficient algorithm for the same.  
\end{enumerate} 

The following claim, which we state without proof (see \cite{DBLP:conf/colt/KlivansS03}) gives us the width of smallest set-multilinear ABP computing any polynomial.
\begin{claim}[Smallest width set-multilinear ABP computing $f$]{\label{claim:smallest_abp_computing_f}}
  Let $f(\mathbf{x})$ be an $n$-variate, degree $d$ polynomial which is set-multilinear in the variable sets $\mathbf{x}_1, \ldots, \mathbf{x}_d$. Further, let $w'$ be the width of the smallest size uniform width set-multilinear ABP with the variable ordering $\mathbf{x}_1, \ldots, \mathbf{x}_d$ computing $f$. Then $\textnormal{Evaldim}_{\mathbf{y}_i}(f) = w'$ where $\mathbf{y}_i = \mathbf{x}_1 \uplus \ldots \uplus \mathbf{x}_i$ for each $i \in [d]$.
\end{claim}

Recall from the proof of Claim~\ref{claim:reordering_layer_spaces} that if $f$ is equivalent to $\IMM_{w,d}$ then $\textnormal{Evaldim}_{\mathbf{y_i}}(f(\mathbf{x})) = w^2$ where $\mathbf{y}_i = \mathbf{x}_1 \uplus \ldots \uplus \mathbf{x}_i$ for all $i \in [d]$. Hence the smallest width uniform width set-multilinear ABP computing $f$ has width $w^2$. The following observation which can be easily verified specifies a width $w^2$ set-multilinear ABP that computes $f$.


\begin{observation}[A width $w^2$ ABP computing $f$]{\label{obs:abp_comp_f}}
          Let $X_1, \ldots, X_d$ be $w \times w$ be full rank linear matrices in the variable sets $\mathbf{x}_1, \ldots, \mathbf{x}_d$ respectively. Consider a a set-multilinear polynomial $f = \textnormal{Trace}(X_1 \cdot X_2 \ldots X_d)$. Then there exists a set-multilinear ABP $A$ of width $w^2$ computing $f$ which is given by $A = Y_1 \cdot Y_2 \ldots Y_d$ with $Y_1 = [X_{11}, \ldots , X_{1w}]$, $Y_i = I_w \otimes X_i$ for all $i \in [2,d-1]$ and $X_d = [X_{d1}^T, \ldots, X_{dw}^T]^T$ where $X_{1i}, X_{dj}$ denotes the $i$-th row and $j$-th column of $X_1$ and $X_d$ respectively, i.e.
          \begin{align*}
            Y_1 = [X_{11}, \ldots, X_{1w}]_{1 \times w^2}\ ;\ \ \
              Y_d = \begin{bmatrix}
              X_{d1}\\
              \vdots \\
              X_{dw} \\
              \end{bmatrix}_{w^2 \times 1} \\ 
        \end{align*}
              $\textnormal{and for } i \in [2,d-1]$,
        \begin{align*}  X_i = \begin{bmatrix}
              x_{11}^{(i)} &\ldots &x_{1w}^{(i)} \\ 
              \vdots &\ &\vdots \\ 
              x_{w1}^{(i)} &\ldots &x_{ww}^{(i)} \\ 
              \end{bmatrix}_{w \times w}; Y_i = \begin{bmatrix}
              X_i &\ &\ \\ 
              \ &\ddots &\ \\ 
              \ &\ &X_i \\ 
              \end{bmatrix}_{w^2 \times w^2} \\ 
          \end{align*}
\end{observation} 

\begin{fact}[Group of Symmetries of the determinant polynomial]{\label{fact:group_of_sym_det}}Let $X$ be an $n \times n$ symbolic matrix and $\textnormal{det}(X)$ be the determinant polynomial of $X$. If $Y$ is an $n \times n$ matrix with $\textnormal{det}(Y) = \textnormal{det}({X})$, then exactly one of the following holds:
\begin{enumerate}
    \item $Y = A\cdot X\cdot B$ where $A$ and $B$ are $n \times n$ matrices with $AB = I_n$.
    \item $Y = A \cdot X^T \cdot B$ where $A$ and $B$ are $n \times n$ matrices with $AB = I_n$.
\end{enumerate}
\end{fact}

\begin{fact}{\label{fact:independence_prod_polynomials}}
 Let $\{p_i(\mathbf{x}) : i \in [m] \}$ and $\{q_j(\mathbf{y}) : j \in [n] \}$ be two sets of linearly independent polynomials over $\F$ and let $\mathbf{x}$ and $\mathbf{y}$ be disjoint. Then the set of polynomials $\{p_iq_j(\mathbf{x}\mathbf{y}) : i \in [m], j\in [n] \}$ is also linearly independent over $\F$.
\end{fact}
\begin{proof}
    Suppose $\{p_i(\mathbf{x}) : i \in [m] \}$, $\{q_j(\mathbf{y}) : j \in [n] \}$ are linearly independent sets of polynomials but $\{p_iq_j(\mathbf{x}\mathbf{y}) : i \in [m], j\in [n] \}$ is a linearly dependent set of polynomial. 
    \begin{align*}
        &\sum_{\substack{i \in [m] \\ j \in [n]}}a_{ij}p_i(\mathbf{x})q_j(\mathbf{y}) = 0 \\ 
        \implies & \Big(\sum_{j \in [n]}a_{1j} \cdot q_j\Big) p_1 + \ldots + \Big(\sum_{j \in [n]}a_mj \cdot q_j\Big) p_m = 0.\\
        \implies & \sum_{j \in [n]}a_{ij} \cdot q_j = 0\ ;\forall i \in [m]\ (\because p_1,\ldots,p_m \text{ are linearly independent}) \\ 
        \implies & a_{ij} = 0\ ;\forall i \in [m],j \in [n]\ (\because q_1,\ldots,q_n \text{ are linearly independent})
    \end{align*}
 Hence the set of polynomials $\{p_iq_j(\mathbf{x}\mathbf{y}) : i \in [m], j\in [n] \}$ are also linearly independent.
\end{proof}

